Streaming Linear System Identification with Reverse Experience Replay

We consider the problem of estimating a linear time-invariant (LTI) dynamical system from a single trajectory via streaming algorithms, which is encountered in several applications including reinforcement learning (RL) and time-series analysis. While the LTI system estimation problem is well-studied in the {\em offline} setting, the practically important streaming/online setting has received little attention. Standard streaming methods like stochastic gradient descent (SGD) are unlikely to work since streaming points can be highly correlated. In this work, we propose a novel streaming algorithm, SGD with Reverse Experience Replay ($\mathsf{SGD}-\mathsf{RER}$), that is inspired by the experience replay (ER) technique popular in the RL literature. $\mathsf{SGD}-\mathsf{RER}$ divides data into small buffers and runs SGD backwards on the data stored in the individual buffers. We show that this algorithm exactly deconstructs the dependency structure and obtains information theoretically optimal guarantees for both parameter error and prediction error. Thus, we provide the first -- to the best of our knowledge -- optimal SGD-style algorithm for the classical problem of linear system identification with a first order oracle. Furthermore, $\mathsf{SGD}-\mathsf{RER}$ can be applied to more general settings like sparse LTI identification with known sparsity pattern, and non-linear dynamical systems. Our work demonstrates that the knowledge of data dependency structure can aid us in designing statistically and computationally efficient algorithms which can "decorrelate" streaming samples.

==> analysis_of_algorithm.tex <==
%analysis of the algorithm
%\section{Analysis of SGD-RER}
%\label{sec:algorithm_analysis}
%\subsection{Notations}
%\label{subsec:notations}
%Before we analyze this algorithm, we define some notations:
%\begin{\Ieee}{LLL}
%X^t_{-i}=X^t_{(S-1)-i},\, 0\leq i\leq S-1\label{eq:X_minus_i}\Ieeen\\
%\nx=\max_{t\leq T}\norm{X_t}\label{eq:normx}\Ieeen \\
%\Gamma=\sum_{s=0}^{\infty}\A^s (\A^{\top})^s\label{eq:grammian}\Ieeen\\
%\Gamma_t=\sum_{s=0}^{t-1}\A^s (\A^{\top})^s\label{eq:grammian_t}\Ieeen\\
%\hat{\gamma}=4\gamma(1-\gamma\nx^2)\label{eq:gamma_hat}\Ieeen\\
%%\norm{A}\equiv \norm{A}_{\mathrm{op}}\, \mathrm{the\, operator \, norm \, of \, matrix\,} A\Ieeen\\
%\cc^t_{-j}=\left\{\norm{X^{t}_{-j}}^2\leq R\right\}\Ieeen\label{eq:Ct_event}\\
%\cct^{t}_{-j}=\left\{\norm{\tilde X^{t}_{-j}}^2\leq R\right\}\Ieeen\label{eq:Ct_tilde_event}\\
%\cd^t_{-j}=\left\{\norm{X^{t}_{-i}}^2\leq R:\,j\leq i\leq B-1\right\}=\bigcap_{i=j}^{B-1}\cc^t_{-i}\sk{\, check\, R\, defn\,}\label{eq:Dt_Event}\Ieeen\\
%\cd^{s,t}=\begin{cases} \bigcap_{r=s}^t \cd^r_{-0} & s\leq t\\
%I & s>t 
%\end{cases}\label{eq:Dst_event}\Ieeen\\
%\tilde\cd^t_{-j}=\left\{\norm{\tilde X^{t}_{-i}}^2\leq R:\,j\leq i\leq B-1\right\}=\bigcap_{i=j}^{B-1}\cct^t_{-i}\sk{\, check\, R\, defn\,}\label{eq:Dt_tilde_Event}\Ieeen\\
%\tilde \cd^{s,t}=\begin{cases} \bigcap_{r=s}^t \tilde \cd^r_{-0} & s\leq t\\
%I & s>t 
%\end{cases}\label{eq:Dst_tilde_event}\Ieeen\\
%\cdh^t_{-j}=\cd^{t}_{-j}\cap \cdt^t_{-j}\label{eq:Dt_both_event}\Ieeen\\
%\cdh^{s,t}=\cd^{s,t}\cap \cdt^{s,t}\label{eq:Dst_both_event}\Ieeen
%\end{\Ieee}





%\input{basic_lemmas}

%As is common in the analysis of least squares regression, we decompose the iterates of $\sgdber$ into bias and variance terms. We obtain the following lemma by using Equation~\eqref{eq:expreplay3}.  Recall the definitions  of `bias' $\Ato{t}{B}$ and `variance' $\Atdiff{t}{B} $ from Equations~\eqref{eq:At0} and~\eqref{eq:Atv}. 
%
%\begin{lemma}[Bias-Variance Decomposition]
%\label{lem:3}
% We have the following decomposition: 
%\begin{\Ieee}{LLL}
%\label{eq:bias_var}
%%\gram{\Atdiff{t}{B}} &\preceq & 3\left[\gram{ \Ato{t}{B}}+\right.\\
%%&&\left. \gram{ \Ata{t}{B}}+\gram{ \Atb{t}{B}} \right]\Ieeen
%\gram{\left(\At{t}{B}-\A\right)} &\preceq &  2\left[\gram{ \Ato{t}{B}}+\right.\\
%&& \left. \gram{ \Atdiff{t}{B}} \right]\Ieeen
%\end{\Ieee}
%
%%\begin{\Ieee}{LLL}
%%\Ato{t}{B}=(A_0-\A)\prod_{s=0}^{t-1}\Ht{s}{0}{B-1} \Ieeen\label{eq:At0}\\
%%\Ata{t}{B}=2\gamma\sum_{r=1}^{t}\sum_{j=0}^{B-1}\Nt{t-r}{-j}\Xt{t-r}{-j}^T \Ht{t-r}{j+1}{B-1}\prod_{s=r-1}^{1}\Htt{t-s}{0}{B-1}\Ieeen \label{eq:At1} \\
%%\Atb{t}{B}=2\gamma\sum_{r=1}^{t}\sum_{j=0}^{B-1}\Nt{t-r}{-j}\Xt{t-r}{-j}^T \Ht{t-r}{j+1}{B-1}\left[{\prod_{s=r-1}^{1}\Ht{t-s}{0}{B-1}}-{\prod_{s=r-1}^{1}\Htt{t-s}{0}{B-1}}\right]\Ieeen \label{eq:At2} \\
%%\end{\Ieee}
%
%
%
%%\sk{unused defn}
%%\begin{\Ieee}{LLL}
%%A^{t,v}_B-A^{t,1}_B&=& 2\gamma\sum_{r=1}^{t}\sum_{j=0}^{B-1}\Nt{t-r}{-j}\left[\Xttr{t-r}{-j}\Ht{t-r}{j+1}{B-1}{\prod_{s=r-1}^{1}\Ht{t-s}{0}{B-1}} \right.\\
%%&&\left. -\Xtttr{t-r}{-j}\Htt{t-r}{j+1}{B-1}{\prod_{s=r-1}^{1}\Htt{t-s}{0}{B-1}}\right]\Ieeen \label{eq:At2} \\
%%\end{\Ieee}
%
%
%\end{lemma}
%We analyze the bias term in Section~\ref{subsec:bias_last_iterate} and the variance term in Section~\ref{subsec:variance_last_iterate}. 
%
%
%We state the informal version of Theorems~\ref{th:1} and~\ref{th:3} here. In the following, we assume that $u,\gamma,B,\alpha$ and $R$ are as chosen in Section~\ref{sec:main_results}. In the following statements, $\tilde{\mathcal{D}}^{0,N-1}$ is an event such that $\mathbb{P}\left(\tilde{\mathcal{D}}^{0,N-1}\right) \geq 1-\frac{1}{T^{\alpha}}$. All the constants below depend only on the sub-Gaussianity parameter $C_{\mu}$ from Assumption~\ref{as:noise_concentration}.
%\begin{theorem}[Informal version of Theorem~\ref{th:1}]
%\begin{\Ieee}{LLL}
%\Ex{\gram{\Atdiff{t}{B}}\indh{0}{N-1}}&\preceq & c_1\left(\gamma \tr(\Sigma)I +  \gamma \tr(\Sigma)  (Bt)^3\norm{\A^u} I\right)\\
%&&+c_2\gamma d\sigma_{\max}(\Sigma)(Bt)^2\prbndsq I\Ieeen
%\end{\Ieee}
%
%\end{theorem}
%For a formal statement we refer to Section~\ref{subsec:variance_last_iterate}. 
%\begin{theorem}[Informal version of Theorem~\ref{th:3}]
%\begin{\Ieee}{LLL}
%\Ex{\gram{\Ato{t}{B}}\indh{0}{N-1}}\preceq \\
%\norm{A_0-\A}^2 \left[\left(1-c_2\gamma B\sigma_{\min}(G)\right)^{t}+\prbnd+c_3\norm{\A^u}\right]I\Ieeen
%\end{\Ieee}
%\end{theorem}
%For a formal statement and proof we refer to Section~\ref{subsec:bias_last_iterate}. 
%
%\subsection{Tail-averaged iterate}
%
%Our main goal is to understand the performance (estimation and prediction) of the tail-averaged iterate.
%\begin{\Ieee}{LLL}
%\label{eq:tail_avg_iterate}
%\Ana=\frac{1}{N-a}\sum_{t=a+1}^N \At{t}{B}
%\end{\Ieee}
%for $a=\lceil\theta N \rceil$ with $0<\theta <1$. We can decompose the above into bias an variance as 
%\begin{equation}
%\label{eq:tail_bias_var}
%\Ana=\Anav+\Anab
%\end{equation}
%with
%\begin{\Ieee}{LLL}
%\Anav=\frac{1}{N-a}\sum_{t=a+1}^N \Av{t}{B}\Ieeen\label{eq:tail_var}\\
%\Anab=\frac{1}{N-a}\sum_{t=a+1}^N \Ab{t}{B}\Ieeen\label{eq:tail_bias}\\
%\end{\Ieee}
%
%
%\begin{proposition}[Informal Version of Proposition~\ref{prop:avg_var1}]
%
%\begin{\Ieee}{LLL}
%&\Ex{\gram{\Anva{a}{N}}\indh{0}{N-1}}\\
%&\preceq \frac{1}{(N-a)^2} \sum_{t=a+1}^N \left[V_{t} \left(I-\ch\right)^{-1}+ \left(I-\ch^{\top}\right)^{-1}V_{t} \right] + \text{ lower order terms}\Ieeen
%\end{\Ieee}
%
%Where,
%\begin{\Ieee}{LLL}
%\ch :=\Ex{\prod_{j=0}^{B-1}\left(I-2\gamma \Xt{0}{-j} \Xttr{0}{-j}\right)1\left[\cap_{j=0}^{B-1}\left\{\norm{\Xt{0}{-j}}^2\leq R\right\}\right]}
%\end{\Ieee}
%$$V_t := \Ex{\gram{\Ato{t}{B}}\indh{0}{N-1}}$$
%
%\end{proposition}
%
%\begin{theorem}[Informal Version of Theorem~\ref{th:4}]
%Let $T = N(B+u)$ and $0<\theta<1$. Then:
%\begin{\Ieee}{LLL}
%\norm{\Ex{\gram{\Anoa{\theta N}{N}}\indh{0}{N-1}}}\leq \\
% \left(c_2\frac{1}{NB(1-\theta)}\frac{e^{-c_3 NB \gamma \sigma_{\min}(G)\theta}}{\gamma \sigma_{\min}(G)} +c_4\left(T\norm{\A^u} +\prbnd\right) \right)\norm{A_0-\A}^2 \Ieeen
%\end{\Ieee}
%\end{theorem}
%
%We finally combine these ingredients to bound the prediction error $\losspred(\hat{A}_{\theta N,N})$ in Sections~\ref{sec:pred_var} and~\ref{sec:pred_bias}. Here, we use the following technical lemma to ensure that we obtain the optimal leading order dependence of $\frac{d\tr(\Sigma)}{T}$, without any condition number factors contained in $G$ which can in general depend on the spectral radius $\rho(\A)$. 
%
%\begin{lemma}[Informal Version of Lemma~\ref{lem:H_plus_HT_bound}]
%Let $\gamma\leq \frac{1}{8RB}$. Then 
%\begin{\Ieee}{LLL}
%\ch +\ch^{\top} \preceq 2\left(I-\frac{4}{3}\gamma B G\right)+\frac{8}{3}\gamma B\sqrt{M_4}\prbndsq I \Ieeen
%\end{\Ieee} 
%where $M_4=\Ex{\norm{\Xtt{0}{-0}}^4}$. 
%\end{lemma}
%We develop the theory behind the proof of Theorem~\ref{thm:main_upper_bound_op} on similar lines in Section~\ref{sec:op_norm}, with the difference that we obtain high probability bounds via. Chernoff bound and $\epsilon$-net arguments.

%$\Ata{t}{B},\Atb{t}{B}$ capture the uncertainty due to the inherent noise in the data. Their sum can be viewed as the output of $\sgdber$ when started at the optimal $\A$. 

%\input{last_iterate_analysis}
%\input{average_iterate_analysis}
%\input{bias_analysis}
%\input{prediction_variance}
%\input{prediction_bias}

==> conc.tex <==
\section{Conclusions}
\label{sec:conc}

==> formal_results.tex <==
%%Formal statement of the results
%\section{Formal Statement of Results}
%\label{sec:formal_results}
%For all the results below, we suppose that Assumptions~\ref{as:norm_condition},~\ref{as:noise_concentration} and~\ref{as:stationarity} hold.
%\begin{theorem}\label{thm:main_upper_bound_op}
%Suppose $R,B,\alpha$ and $u$ are chosen chosen in Section~\ref{sec:main_results}. Suppose we pick the step size $\gamma < \min \left(\tfrac{C}{B\lmin{G}},\tfrac{1}{8BR}\right)$ for some constant $C$ depending only on $C_{\mu}$. Let $\hat{A}_{a,N}$ be the tail averaged output of $\sgdber$ with $T$ data points as defined in Equation~\eqref{eq:tail_average_definition}. Let $\upsilon > 1$ be such that $\upsilon < \alpha/2 - 1$
%Then, with probability at least $1-\frac{1}{T^{\upsilon}}$, we have:
%$$
%\lossop(\hat{A}_{a,N},\A,\mu) \leq C\sqrt{\frac{(d+\upsilon\log T) \lmax{\Sigma}}{N B  \lmin{G}} }  + \beta_{b} + \beta_{1,v}$$
%Where:
%\begin{align*}
%\beta_b &= T^{\upsilon}\sqrt{d}\left(\frac{c_2e^{-c_3 a B \gamma \sigma_{\min}(G)}}{\sqrt{(N-a)B\gamma \sigma_{\min}(G)}}+c_4\left(\sqrt{T\norm{\A^{u}}} +\frac{1}{T^{\alpha/2}}\right) \right)\norm{A_0-\A}
%\end{align*}
%
%$$ \beta_{1,v} =C T^{\upsilon}  \sqrt{d\gamma \tr(\Sigma)}  (Bt)^2\norm{\A^u} $$
%\end{theorem}
%The techniques for the proof is developed in Section~\ref{sec:op_norm} and the Theorem~\ref{thm:main_upper_bound_op} is proved in Section~\ref{sec:main_op_bound}.
%\begin{theorem}\label{thm:main_upper_bound_pred}
%Let $R,B,u$ and $\alpha$ are chosen as in section~\ref{sec:main_results}. Let $\gamma \leq \min\left\{\frac{c}{6RB},\frac{1}{2R}\right\}$ for $0<c<1$. 
% Then there are constants $\{c_i>0:1\leq i\leq 2\}$ such that for $\prbndsqinv>c_1\frac{\sqrt{M_4}}{\sigma_{\min}(G)}$  the conditional expected prediction error is bounded as 
%\begin{\Ieee}{LLL}
%\Ex{\losspred(\hat A_{\theta N,N};\A,\mu)\ind{0}{N-1}}\leq \tr(\Sigma) +c_2\frac{d\tr(\Sigma)}{NB(1-\theta)}+\\
%c_3\frac{1}{NB(1-\theta)}\frac{ d\kappa(G)}{\gamma }e^{-c_4 NB \gamma \sigma_{\min}(G)\theta}\norm{A_0-\A}^2+\\
%\norm{\A^u}e^{c_4\left(\log(T)+\log\left(\frac{\sigma_{\max}(\Sigma)}{\sigma_{\max}(G)}\right)+\log\norm{ A_0-A^* }^2\right)}+\frac{d^2\sigma_{\max}(\Sigma)}{NB}o(1)\Ieeen
%\end{\Ieee}
%
%where $o(1)\to 0$ as $T\to\infty$ that contain terms that depend on $R,d,G,\Sigma,\gamma, A_0$, and 
%$$\cd^{0,N-1}=\left\{\norm{\Xt{t}{-j}}^2\leq R: 1\leq t\leq N-1,\, 0\leq j\leq B-1\right\}$$
%with $\Pb{\cd^{0,N-1}}\geq 1-\prbnd$
%\end{theorem}
%
%The proof of the above theorem is provided in the appendix in sections~\ref{sec:pred_var} and \ref{sec:pred_bias}. In particular, the result follows by combining theorems~\ref{thm:predloss_vari} and \ref{thm:pred_bias}.

==> setting_the_gap.tex <==
% setting the parameter u


\section{Setting the Buffer Gap}
\label{sec:setting_u}



 They key problem dependent parameter in the Algorithm is $u$. We have the Gelfand formula for spectral radius which shows that $\lim_{k\to \infty}\|\A^k\|^{1/k} = \rho(\A)$. Now, if $\A$ is such that $\rho(\A)<1$ but $\|\A\|>1$ (a case studied by \citep{simchowitz2018learning}), then we need to make $u$ as large as $C d\log T$ which would lead to a relatively large buffer size $B$ of $d\log T$. To see this, we verify the proof by \citep{petrovgelfand} (by replacing $A$ with $\frac{A}{\|A\|}$ and $\rho(A)$ with $\frac{\rho}{\|A\| }$ in the proof) to show that $\|\A^{k}\| \leq \left(2k\|\A\|\right)^d\rho^{k-d}  $ whenever $k \geq d$. Therefore, in the worst case, we can pick $u = O\bigr(\left(\log \left(T\lmax{G}\right) + d\log d\|A\| \right)/\log 1/\rho\bigr)$.

\begin{remark}
In the case of $\rho<1$ but $\norm{\A}>1$, $\kappa(G)$ can grow super linearly in $d$. For instance, consider $\A$ to be nilpotent of order $d$ (i.e. $\A^{d-1}\neq 0$ but $\A^d=0$). Here $\sigma_{\max}(G)$ can grow like $\norm{\A}^d$. So we need exponentially (in $d$) many samples for bias decay.
\end{remark}


%So, for the rest of the discussion we focus on setting where $\rho(A)\leq \|A\|<1$. We first discuss the more widely applicable  and interesting case where $\|A\|\leq c<1$ and $c$ is a constant. In this case, we can set $u=\log T$. Here, we make the following observations: 

%\begin{enumerate}
%\item Setting $a=\log T$ , we get that $t\cdot B\geq \frac{C}{\log T} t \cdot S$ where $t\cdot S$ is the total number of point observed till $t$-th buffer and $C$ is a constant. Furthermore, The total buffer size $S=B+u$ scales only logarithmically with respect to $T$ and is independent of $d$. So, the algorithm has nearly {\em linear} (in $d$) buffer space complexity (since we are storing length $d$ vectors) and linear (in terms of number of parameters) time complexity. \label{item:1}%\theta N$ with either i) $\theta=\frac{\log T}{N}$ or ii) constant $\theta\in (0,1)$, we get that $(N-a)B \geq C T$ for some constant $C>0$. \label{item:1}\\
%\item Bound on $\lossop$: following item \ref{item:1} above, our asymptotic variance bound matches the information theoretically optimal bound (up to logarithmic factor) for the $\var(\A,\mu)$ estimation problem \citep{simchowitz2018learning}, and is in fact stronger than the bound of offline OLS by \citep{simchowitz2018learning}. 
%\item SGD for linear regression with {\em independent} data \citep{jain2017parallelizing,defossez2015averaged}, but with similar problem setting incurs error  $O(\sqrt{\frac{d Tr(G^{-1}\Sigma)}{T}})$. So  our bound for $\sgdber$ matches the independent data setting bound in the minimax sense but is worse in terms of problem-dependent parameters $G$ and $\Sigma$. We leave further investigation into better error dependence on $G$ and $\Sigma$ for future work. 
%
%\item Bound on $\losspred$: Again from item \ref{item:1}, the leading term matches the information theoretic lower bound in theorem~\ref{thm:main_lower_bound} in terms of the dependence on $T$ and $d$. Note that for the choice of $B$ in the beginning of this section, the term $\frac{\sqrt{\kappa(G)}}{B}$ is $o(1)$ and can be ignored.
%\end{enumerate}

%\begin{enumerate}
%\item As in the previous case, our error bounds are minimax optimal (up to logarithmic factors). Furthermore, in this case, we require $a=\Omega(T^{\xi})$ and need $B=\Omega(T^{\xi})$ since $\log(1/\norm{\A})\geq \frac{1}{T^{\xi}}$. Hence $N=O(T^{1-\xi})$ which implies that $\theta$ in the Algorithm~\ref{alg:1} is of the order $\frac{1}{T^{1-2\xi}}$.
%\item Since $\sigma_{\max}(G)=O(T^{\xi})$, the exponential bias term in both the bounds above (see theorem~\ref{thm:main_upper_bound_pred} for the bias term in prediction error) will not decay if $\xi\geq 1/2$.
%\end{enumerate}

\begin{remark}
In the case of $\rho<1$ but $\norm{\A}>1$, $\kappa(G)$ can grow super linearly in $d$. For instance, consider $\A$ to be nilpotent of order $d$ (i.e. $\A^{d-1}\neq 0$ but $\A^d=0$). Here $\sigma_{\max}(G)$ can grow like $\norm{\A}^d$. So we need exponentially (in $d$) many samples for bias decay.
\end{remark}

==> sgd_shortcomings.tex <==
%sgd shortcomings


\section{Shortcomings of SGD}
\label{sec:normal_sgd}
